An investigation of security controls and MITRE ATT\&CK techniques

Attackers utilize a plethora of adversarial techniques in cyberattacks to compromise the confidentiality, integrity, and availability of the target organizations and systems. Information security standards such as NIST, ISO/IEC specify hundreds of security controls that organizations can enforce to protect and defend the information systems from adversarial techniques. However, implementing all the available controls at the same time can be infeasible and security controls need to be investigated in terms of their mitigation ability over adversarial techniques used in cyberattacks as well. The goal of this research is to aid organizations in making informed choices on security controls to defend against cyberthreats through an investigation of adversarial techniques used in current cyberattacks. In this study, we investigated the extent of mitigation of 298 NIST SP800-53 controls over 188 adversarial techniques used in 669 cybercrime groups and malware cataloged in the MITRE ATT\&CK framework based upon an existing mapping between the controls and techniques. We identify that, based on the mapping, only 101 out of 298 control are capable of mitigating adversarial techniques. However, we also identify that 53 adversarial techniques cannot be mitigated by any existing controls, and these techniques primarily aid adversaries in bypassing system defense and discovering targeted system information. We identify a set of 20 critical controls that can mitigate 134 adversarial techniques, and on average, can mitigate 72\% of all techniques used by 98\% of the cataloged adversaries in MITRE ATT\&CK. We urge organizations, that do not have any controls enforced in place, to implement the top controls identified in the study.

==> backup.tex <==
\subsubsection{Risk}
Organizations enforce security controls to mitigate risks from potential cyberthreats. In this study's scope, adversarial techniques pose risks, and security controls reduce or eliminate risk through mitigating adversarial techniques. Hence, we can measure the extent of risk mitigation of security controls by measuring the risk incurred by the mitigated techniques. We use the generic equation: $risk = likelihood \times severity ~\refstepcounter{equation}(\theequation)\label{eq-risk}$ from ~\cite[p.~13]{hubbardHowMeasureAnything2016} to measure the risk of adversarial techniques. We approximate the $likelihood$ of a technique by computing the fraction of adversary entities that use the technique. However, we also require to approximate how \textit{severe} an adversarial technique is. We provide an example followed by the equation on how we approximate the severity of adversarial techniques below. 

Fig.~\ref{fig:riskExample} shows a real-world example of adversaries using techniques to launch cyberattacks. A cybercriminal group named admin@338~\cite{admin338} uses three following techniques: (a) \textit{T1059: Command and scripting interpreter}~\cite{}; (b) \textit{T1566: Phishing}~\cite{}; and (c) \textit{T1204: User execution}~\cite{}. Another cybercriminal group named APT-C-36~\cite{aptC36} uses three following techniques: (a) \textit{T1059: Command and scripting interpreter}~\cite{}; (b) \textit{T1027: Obfuscated file or information}~\cite{}; and (c) \textit{T1105: Ingress tool transfer}~\cite{}. We observe that adversaries used \textit{T1059} technique with four different adversarial techniques. As adversaries use techniques to achieve tactical goals toward breaching a system, we assume that techniques used in conjunction with many other techniques are relatively more severe. For example, an adversary can perform a plethora of malicious operations through \textit{T1059: Command and scripting interpreter}, such as executing malicious code or transferring confidential files to remote. In the figure, we also observe adversaries use the technique in conjunction with other techniques such as phishing and user execution. Adversaries often perform one technique to be able to perform another one to gain tactical objectives. For example, the figure shows that an adversary first performs \textit{T1566: phishing} to trick users into \textit{T1204: user execution} of malicious code. Hence, given that adversary uses \textit{T1566: phishing}, the adversary may use \textit{T1204: user execution} technique.

From the example, we observe two severity perspectives of a given technique: (a) the number of techniques used in conjunction with the technique; and (b) how probable an adversary is to use the technique in conjunction with other techniques. On the right side of the figure, we build a graph showing the severity perspective of \textit{T1059} and \textit{T1566}. In the graph, a node represents a technique, and an edge represents two techniques used in conjunction. The degree count of \textit{T1059} and \textit{T1566} are four and two, respectively, indicating the number of other techniques used in conjunction. The labels on the four outgoing edges of \textit{T1059} show the likelihood of conjunction given that an adversary uses \textit{T1059}.  

We use the following equation to measure the severity(SV) of a technique $te$ : $SV(te) = e^{-h/\alpha} \times C~\refstepcounter{equation}(\theequation)\label{eq-severity}$ adopted from~\cite{hadarCyberDigitalTwin2020}. Here, $C$ denotes the degree count of $te$. $h$ denotes the mean of $1-p_i$ where
$te$ is used in conjunction with $n$ other techniques, and $p_i$ is the likelihood of the conjunction of $i^{th}$ among the $n$ other techniques. $\alpha$ is a constant, and we set $\alpha = 8$ as mentioned in~\cite{hadarCyberDigitalTwin2020}. We provide an example of the equation from the figure. The degree count of \textit{T1059} is 4, and four techniques are used in conjunction with a likelihood of 0.5 each. Hence, $h = \frac{(1-0.5) + (1-0.5) + (1-0.5) + (1-0.5)}{4} = 0.5$, and $SV(T1059) = e^{-0.5/8} \times 4 = 3.76$. The degree count of \textit{T1566} is 2, and two techniques are used in conjunction with a likelihood of 1.0 each. Hence, $h = \frac{(1-1) + (1-1)}{2} = 0$, and $SV(T1566) = e^{-0/8} \times 2 = 2$ . 

\textbf{Control's Mitigated Risk (CMR):} The mitigated risk (CMR) by a control $c$ refers to the risk of the mitigated techniques.  Hence, $CMR(c) = \sum_{i=0}^{n} R(te_i)~\refstepcounter{equation}(\theequation)\label{eq-risk2}$ where $c$ mitigated $n$ techniques: $te_1, te_2, ..., te_n$, and $R(te_i)$ is the risk of $i^{th}$ mitigated technique $te_i$. We compute $R(te_i)$ by the following equation: $R(te_i) = LK(te_i) \times SV(te_i)~\refstepcounter{equation}(\theequation)\label{eq-risk3}$. Here, $LK(te_i)$ is the likelihood of the technique $te_i$, which is the fraction of adversaries using $te_i$. $SV(te_i)$ is the severity of $te_i$. We provide an example based on the figure. Assume two controls $c_1, c_2$ where $c_1$ mitigates \textit{T1059} and \textit{T1566}, and $c_2$ mitigates \textit{T1566}. Hence, $CMR(c_1) = R(T1059) + R(T1566)$, and $CMR(c_2) = R(T1566)$. Both the two adversaries use \textit{T1059}, and hence, $LK(T1059) = 1$. Hence, $R(T1059) = LK(T1059) \times SV(T1059) = 1 \times 3.76 = 3.76$. One out of the two adversaries use \textit{T1566}, and hence, $LK(T1566) = 0.5$. Hence, $R(T1566) = LK(T1566) \times SV(T1566) = 0.5 \times 2 = 1$. Hence, $CMR(c_1) = R(T1059) + R(T1566) = 4.76$, and $CMR(c_2) = R(T1566) = 1$. 

\textbf{Summary of the metrics:} Overall, we introduce six metrics to measure the defensive capabilities of security controls. In Table~\ref{tab:metrics}, we discuss the practical implication of the metrics. 

\begin{table*}[]
    \centering
    \scriptsize
    \caption{Practical implication of the introduced metrics}
    \label{tab:metrics}
    \begin{tabular}{p{3cm}p{14cm}}
    \toprule
    \textbf{Metric} & \textbf{Implication} \\ \midrule
    
        CV-1: Technique Coverage (TEC) & TEC indicates how many techniques a control can mitigate. A relatively higher TEC of a control indicates that the control mitigates a relatively higher number of techniques. Organizations can achieve protection against a relatively high number of adversarial techniques by implementing controls with high TEC \\ \midrule
        
        CV-2: Tactic Coverage (TAC) & TAC indicates how many techniques of a given tactic a control can mitigate. A relatively higher TAC of a control and a given tactic indicates that the control mitigates a relatively higher number of techniques of the tactic. An adversary can use multiple techniques of the same tactic to achieve the tactical goal. For example, ATT\&CK catalogs 13 techniques that can aid an adversary in gaining the objective of \textit{TA0004: Privilege escalation}~\cite{}. Hence, a control having a relatively higher TAC value for \textit{TA0004: Privilege escalation} tactic can aid organizations in gaining relatively higher protection against privilege escalation attempts from adversaries. \\ \midrule
        
        CV-3: Mean Tactic Coverage (MTAC) & MTAC reflects a control's overall mitigation of techniques from all 14 tactics cataloged in ATT\&CK. A higher value in MTAC indicates the control mitigates a relatively higher number of techniques from all 14 tactics. Hence, organizations can achieve protection against a relatively high number of adversarial techniques across all 14 tactics by implementing controls with high MTAC \\ \midrule
        
        CV-4: Adversary Entity Coverage (AC) & AC reflects how relevant a control is against all the cataloged adversary entities in ATT\&CK. A relatively higher value indicates that the control can be effective against a relatively higher number of adversaries. Organizations can achieve protection against a relatively high number of adversaries by implementing controls with high AC  \\ \midrule
        
        CV-5: Adversary Entity Technique Coverage (ATC) & A control can mitigate multiple techniques, and an adversary can use multiple techniques. Hence, ATC reflects the mean percentage of mitigated techniques used by all cataloged adversaries in ATT\&CK. Organizations can achieve protection against a relatively high percentage of techniques of all adversaries by implementing controls with high ATC  \\ \midrule
        
        RD-1: Control Redundancy (CR) & CR reflects how important a control is for mitigating techniques from the perspective of available alternative controls. A relatively lower value indicates that the control has a relatively lower number of alternatives. Organizations may require to enforce the control and ensure that control does not fail \\ \midrule
        
        RS-1: Control's Mitigated Risk (CMR) & CMR reflects the risk mitigation capability of a control. Organizations can mitigate a relatively higher amount of risk by implementing controls with a relatively higher CMR \\ 
    \bottomrule
    \end{tabular}
\end{table*}

